Detailed compositional analysis of the heavily polluted DBZ white dwarf SDSS J073842.56+183509.06: A window on planet formation?

We present a new model atmosphere analysis of the most metal contaminated white dwarf known, the DBZ SDSS J073842.56+183509.06. Using new high resolution spectroscopic observations taken with Keck and Magellan, we determine precise atmospheric parameters and measure abundances of 14 elements heavier than helium. We also report new Spitzer mid-infrared photometric data that are used to better constrain the properties of the debris disk orbiting this star. Our detailed analysis, which combines data taken from 7 different observational facilities (GALEX, Gemini, Keck, Magellan, MMT, SDSS and Spitzer) clearly demonstrate that J0738+1835 is accreting large amounts of rocky terrestrial-like material that has been tidally disrupted into a debris disk. We estimate that the body responsible for the photospheric metal contamination was at least as large Ceres, but was much drier, with less than 1% of the mass contained in the form of water ice, indicating that it formed interior to the snow line around its parent star. We also find a correlation between the abundances (relative to Mg and bulk Earth) and the condensation temperature; refractory species are clearly depleted while the more volatile elements are possibly enhanced. This could be the signature of a body that formed in a lower temperature environment than where Earth formed. Alternatively, we could be witnessing the remains of a differentiated body that lost a large part of its outer layers.

==> tab1.tex <==
\begin{deluxetable}{lccccc}
\tabletypesize{\scriptsize}
\tablecolumns{11}
\tablewidth{0pt}
\tablecaption{Stellar parameters adopted for SDSS J0738+1835}
\tablehead{Parameter & Value}
\startdata
$T_{\rm eff}$(K)  & 13950 $\pm$ 100    \\
$\log g$         & 8.4 $\pm$ 0.2    \\
$M_{\rm WD}/M_{\odot}$     & 0.841  $\pm$ 0.131  \\
$M_{\rm init}/M_{\odot}$  &   4.47 $\pm$0.36 $^a$  \\
$R/R_{\odot}$     & 0.00958 $\pm$ 0.0015  \\
$\log L/L_{\odot}$ & $-$2.50 $\pm$0.12 \\
$D$              & 147 pc $\pm$23 \\
Cooling Age      & 477 Myr $\pm$ 160\\
$\log (M_{\rm He}/M_{\star})$ &  $-$6.41 $+0.56$/$-0.28$ \\
\enddata
\tablenotetext{a}{Initial mass of the main sequence progenitor
  calculated using the Initial-Final Mass Relation of
  \citet{williams09}}
\end{deluxetable}



==> tab2.tex <==
\begin{deluxetable}{lccccc}
\tabletypesize{\scriptsize}
\tablecolumns{11}
\tablewidth{0pt}
\tablecaption{}
\tablehead{Element & log $[n(Z)/n(He)]_{phot}$  & $M_{\rm CVZ}/(10^{21}$g) & log $\tau_{set}$(yr) & $[n(Z)/n(Fe)]_{acc}$ & $\dot M /(10^8g~s^{-1})$ }
\startdata

1  ~H & -5.73 $\pm$ 0.17 & 0.310  & $\infty$ &  \ldots & \ldots \\
8  ~O & -3.81 $\pm$ 0.19 & 407.86 & 5.244 & 9.52 & 740.2 \\
11 Na & -6.36 $\pm$ 0.16 & 1.639  & 5.238 & $2.7\times 10^{-2}$ & 3.02 \\
12 Mg & -4.68 $\pm$ 0.07 & 83.33 & 5.258 & 1.24 & 146.38 \\
13 Al & -6.39 $\pm$ 0.11 & 1.792 & 5.244 & $2.5\times 10^{-2}$  & 3.25\\
14 Si & -4.90 $\pm$ 0.16 & 57.99 & 5.248 & 0.77 & 104.36 \\
20 Ca & -6.23 $\pm$ 0.15 & 3.907 & 5.044 & $5.8\times 10^{-2}$ & 11.24 \\
21 Sc & -9.55 $\pm$ 0.18 & 2.05$\times 10^{-3}$ & 5.010 & $2.9\times 10^{-5}$& 6.38$\times 10^{-3}$ \\
22 Ti & -7.95 $\pm$ 0.11 & 8.87$\times 10^{-2}$ & 5.007 & $1.2\times 10^{-3}$  & 0.278 \\
23 V  & -8.50 $\pm$ 0.17 & 2.65$\times 10^{-2}$ & 5.006 & $3.4\times 10^{-4}$ & 8.31$\times 10^{-2}$\\
24 Cr & -6.76 $\pm$ 0.12 & 1.492 & 5.026 & $1.8\times 10^{-2}$ & 4.48 \\
25 Mn & -7.11 $\pm$ 0.11 & 0.693 & 5.028 & $7.7\times 10^{-3}$ & 2.07 \\
26 Fe & -4.98 $\pm$ 0.09 & 94.91& 5.047 & 1.00 & 271.32 \\
27 Co & -7.76 $\pm$ 0.19 & 0.165 & 5.042 & $1.7\times 10^{-3}$ & 0.479 \\
28 Ni & -6.31 $\pm$ 0.10 & 4.721 & 5.063 & $4.6\times 10^{-2}$ & 12.997 \\
\hline
\hline
 &           &          &  &  &  \\
Total &           & 658.95   &  &  & 1301.7 
\enddata
\end{deluxetable}


